A Survey on Large Language Models in Multimodal Recommender Systems

Multimodal recommender systems (MRS) integrate heterogeneous user and item data, such as text, images, and structured information, to enhance recommendation performance. The emergence of large language models (LLMs) introduces new opportunities for MRS by enabling semantic reasoning, in-context learning, and dynamic input handling. Compared to earlier pre-trained language models (PLMs), LLMs offer greater flexibility and generalisation capabilities but also introduce challenges related to scalability and model accessibility. This survey presents a comprehensive review of recent work at the intersection of LLMs and MRS, focusing on prompting strategies, fine-tuning methods, and data adaptation techniques. We propose a novel taxonomy to characterise integration patterns, identify transferable techniques from related recommendation domains, provide an overview of evaluation metrics and datasets, and point to possible future directions. We aim to clarify the emerging role of LLMs in multimodal recommendation and support future research in this rapidly evolving field.

==> MRS_methods/Graphs.tex <==
\subsection{Involved graphs.}
\label{sec:graphs}
In \cite{MRS1_survey}, we can find a distinction among the methods based on fusion, bridge and pruning. The first one refers to inter-relationship between users and items and the second to intra-relations among the items, while the last one refers to pruning process in the user-item relations. This can be considered as collaborative, content based, and collaborative pruning. We will not go in deep into this split, but we will do a general classificcation in the same direction. We will conside rthe graphs involved in the different papers. Considering \GUI as teh graph betweeb users and items, working with it would mean some level of collaborative approach. While using \GII or \GUU, would involve some level of content based point of view in the approach. We add to this classication \textbf{KG}, which are the most common type of graph involved in MRS from outside of the users and items information.

\subsubsection{User-Item Graph}
\paragraph{\GUI}
\cite{HLLM2024}, through LLM agents with predefined prompt structures combined with reasoning prompt techniques that interact with the graph representation.
CTRL \cite{CTRL2023} approaches CTR recommendation by introducing a user and the interacted items as tuples. These tuples have two representations: a text for the LLM and a tabular one for the Collaborative Model. They do not make explicit use of the graph structure. TMF \cite{TripletFusion2024} combines \GUI with other modalities into a graph and then introduces it to the LLM through soft prompting. PPL \cite{PersonalizedPromptLearning} introduces the local information from the \GUI graph without mentioning it explicitly through prompting techniques. In iLoRA \cite{iLoRA}, they treat the users and the items from \GUI in a next-item prediction task as different modalities to be aligned through the proposed combination of LoRA and MoE. 

\subsubsection{Inter-items and inter-users}
\paragraph{\GII and \GUU}

\subsubsection{External Knowledge Graph}
\paragraph{\textbf{KG}}
In some cases, the KG can be used to introduce external knowledge and for training objectives. For example, MMGCL \cite{MMGCL2022} combines \GUI with a KG and masks modalities and edges to apply Contrastive learning.




==> future/conclusion.tex <==
\section{Conclusion}
Our main conclusion is...
Mention that some of the works that we are going to present here are not MRS but SRS, since the attention became a common tool in this branch of RS, where transformers architectures are more advanced \cite{} and specialised \cite{PositionalEncodingSRS, SASRec, CARCA}.

==> others/test.tex <==
\begin{abstract}
Item representation learning (IRL) plays an essential role in recommender systems, especially for sequential recommendation. Traditional sequential recommendation models usually utilize ID embeddings to represent items, which are not shared across different domains and lack the \textit{transferable} ability. Recent studies use pre-trained language models (PLM) for item text embeddings (text-based IRL) that are universally applicable across domains. However, the existing text-based IRL is unaware of the important collaborative filtering (CF) information. In this paper, we propose CoWPiRec, an approach of \underline{Co}llaborative \underline{W}ord-based \underline{P}re-trained \underline{i}tem representation for \underline{Rec}ommendation. To effectively incorporate CF information into text-based IRL, we convert the item-level interaction data to a word graph containing word-level collaborations. Subsequently, we design a novel pre-training task to align the word-level semantic- and CF-related item representation. Extensive experimental results on multiple public datasets demonstrate that compared to state-of-the-art transferable sequential recommenders, CoWPiRec achieves significantly better performances in both fine-tuning and zero-shot settings for cross-scenario recommendation and effectively alleviates the cold-start issue.
\end{abstract}

\section{Methodology}
In this section, we present our proposed transferable item representation learning approach, CoWPiRec.
Utilizing the word-level CF knowledge learned from the co-click word graph, CoWPiRec generates item representation with both semantic and CF-related information based on item text.
When transferring to a new domain, the enhanced item representation could directly perform recommendations without training procedure and contribute to the in-domain training.
\subsection{Framework Overview}
The overall framework of our proposed text-based IRL approach is shown in Figure~\ref{fig_model}.
Text-based IRL approach utilizes item text representation generated by PLM to replace the ID-based item representation of traditional sequential recommendation models. 
It has achieved promising transferable recommendation performance combined with a pre-training scheme on the SRL module~\cite{ding2021zero,hou2022towards}. 
We argue that these transferable recommenders are suboptimal since the text-based IRL modules are unaware of CF-related information and it is desired to incorporate CF-related signals into PLM.

Considering PLM is typically trained with the word-level task, the item-level next-item-prediction task is not applicable to integrate CF signals into PLM.
Therefore, we first extract word pairs with co-click relationships from interaction data and construct a word graph that contains these relationships.
The co-click relationships between these words can be seen as word-level CF signals.
Then we incorporate the word-level CF signals from the word graph into PLM through a word-level pre-training task.
We will explain each key component of our proposed approach in the following sections.

\subsection{Word Graph Construction}
In this section, we present the process of extracting co-click words and constructing the word graph. A sub-graph of our constructed word graph is shown in Figure~\ref{fig_model} (a). The co-click relationship is a common concept in recommender systems while previous works mostly focus on item-level co-click relationships.
To align with the modeling format of PLM and incorporate the recommendation signal more effectively, we extract the word-level co-click relationships from the item text.

In different recommendation scenarios, although items have different presentation formats, they usually have basic textual descriptions.
Due to the universality of language, different domains share a common vocabulary, making the text bridge different recommendation scenarios. 
Additionally, item texts often contain some word-level user preferences. 
If a user clicks several items containing words like ``health” or ``fitness”, it indicates that this user may be focused on a healthy lifestyle.
Therefore, the user may be also interested in nutritionally balanced food or some fitness equipment. 
These items may contain words such as ``balance”, ``exercise” and ``cycling”. 

We construct a word graph to organize the co-click relationships based on user interaction. 
For each word, a candidate set of words is generated based on co-click relationships and then filtered to retain only the top $N$ words as neighboring nodes.

Specifically, given a user's interaction sequence $s=\{i_1,i_2,i_t,...,i_n\}$, where $i_t$ represents the $t$-th item in the sequence. 
A co-click word pair is defined as two words from each item text respectively, denoted as $w_i$ and $w_j$. 
We count the occurrences of all co-click word pairs, denoted as $(w_i, w_j, c_{ij}, c_{ji})$, where $c_{ij}=c_{ji}$. 
Since each word contains a large number of co-click words, we follow~\cite{shi2021wg4rec} and filter the candidate co-click words using the $tf\mbox{-}idf$ algorithm. 
The $tf\mbox{-}idf$ value of a pair of co-click words is calculated by Equation~\eqref{tf-idf}:
\begin{equation}
\begin{gathered}
\label{tf-idf}
    tf_{i,j}=\frac{c_{i,j}}{\sum_{k=1}^{V} c_{i,k}}, \quad idf_{j}=\lg \frac{V}{\left|\left\{c_{k,j} \mid \forall k, c_{k,j}>0\right\}\right|}, \\
    tf\mbox{-}idf_{i,j} = tf_{i,j}\times idf_{j},
\end{gathered}
\end{equation}
where $V$ is the vocabulary size, and the denominator of $idf$ is the number of words that have the co-click relationship with $w_j$. 
The higher the $tf\mbox{-}idf$ value, the more times $w_j$ and $w_i$ are co-clicked and the less $w_j$ is co-clicked with other words. 
For each $w_i$, only the top $N$ words with the highest $tf\mbox{-}idf$ values will be selected as its neighbor nodes in the word graph.

By constructing edges between co-click word pairs, we obtain a word graph fusion of word-level CF signals.
We construct the word graph based on the user interaction data of multiple domains to improve the generality ability of extracted word-level CF signals. The word pairs with edges in the word graph may relate to different domains, e.g. ``health” and  ``balance” in the ``Food” domain, ``cycling”, ``indoor” and ``exercise” in the ``Home” domain, as shown in Figure~\ref{fig_model} (a).

\subsection{Word Graph-based Pre-training Task}
With the remarkable semantic representation ability of PLM, text-based IRL based on PLM provides an effective semantic matching ability.
While PLM cannot capture CF-related information and this limits the representation ability of text-based IRL. 
To incorporate the recommendation signal into PLM, an intuitive idea is to train PLM and SRL simultaneously via the next item prediction task, thus introducing task-specific information into PLM. 
However, since PLM's modeling method on large-scale corpora is word-level, the above item-level supervision signal cannot be well integrated into PLM. 

Considering many works have demonstrated that aligning with PLM's modeling format in downstream tasks can better inspire its learned knowledge~\cite{liu2023pre}, we propose a word-level pre-training task to incorporate the word-level CF information contained in the word graph into the PLM, as shown in Figure~\ref{fig_model} (b).
Specifically, we use item text as the input of the PLM and add special symbols [CLS] and [SEP] before and after the input in accordance with the input format of the PLM. 
We randomly mask words in the item text using the [MASK] special symbol. 
For an item text input $i=\{cls, w_1,...,w_m,...,w_n, sep\}$, where $w_m$ is the masked word, the initialize word embedding of each word is obtained with PLM's word embedding, i.e., $\{\mathbf{v}_{cls}, \mathbf{v}_{1},..., \mathbf{v}_{m},..., \mathbf{v}_{n}, \mathbf{v}_{sep}\}$, where $\mathbf{v}_i\in \mathbb{R}^d$ and $d$ is the dimension of word embedding. 
Then two different modeling procedures are performed for input word embedding, namely \textit{semantic modeling} and \textit{word graph modeling}.

\subsubsection{Semantic Modeling} 
In this modeling procedure, the word embedding of each word in item text $\mathbf{v}_i$ is firstly concatenated, i.e., $\mathbf{x}=[\mathbf{v}_{cls}; \mathbf{v}_{1};...; \mathbf{v}_{m};...; \mathbf{v}_{n}; \mathbf{v}_{sep}]\in\mathbb{R}^{n\times d}$, 
where $n$ is the input length and we omit the special token at the head and tail for convenience.
$[;] $ is the concatenation operation.  
Then $\mathbf{x}$ is fed into the $L$-layer Transformer encoder of the PLM. Each Transformer encoder consists of a multi-head self-attention layer and a position-wise feed-forward layer. 
A residual connection and layer normalization are performed in the above two parts. 
We set $\mathbf{x}^0\in\mathbb{R}^{n\times d}$ as the input, and the output after $l+1$-layer Transformer encoder is obtained by Equation~\eqref{trm}.
\begin{equation}
\begin{gathered}
\label{trm}
\mathbf{x}^{l+1} = Trm(\mathbf{x}^{l}) = LN(\mathbf{s}^{l}+FFN(\mathbf{s}^{l})), \\
\mathbf{s}^{l} = LN(\mathbf{x}^{l}+MHAttn(\mathbf{x}^{l})),
\end{gathered}
\end{equation}
where $Trm(\cdot)$ is the Transformer encoder layer, $LN(\cdot)$ is the layer normalization function, $FFN(\cdot)$ is the position-wise feed-forward layer, $MHAttn(\cdot)$ is the multi-head self-attention layer, $\mathbf{s}^{l}\in \mathbb{R}^{n\times d}$ is the output of the multi-head self-attention layer. The output of the last layer is $\mathbf{x}^{L}=[\mathbf{e}_{cls}; \mathbf{e}_{1};...; \mathbf{e}_{m};...; \mathbf{e}_{n}; \mathbf{e}_{sep}] \in \mathbb{R}^{n\times d}$. 

With the self-attention mechanism of the Transformer Encoder, $\mathbf{e}_i\in \mathbb{R}^d$ integrates the contextual information of other words in the item text, which demonstrates effective semantic representation ability in many tasks.
While in the recommendation system, semantic similarity and recommendation relevance are not related, so the PLM is expected to capture additional recommendation signals to improve the recommendation performance.

\subsubsection{Word Graph Modeling} 
In this part, the representation of each word in input $\mathbf{x}$ is obtained by aggregating the embedding of its neighboring nodes through a graph neural network (GNN). 
Specifically, we follow~\cite{shi2021wg4rec} and use the GraphSAGE algorithm~\cite{hamilton2017inductive} to learn a function for aggregating neighbor node representations. 
\begin{equation}
\label{graphsgae}
\mathbf{h}_i^t=\sigma\left(\mathbf{W}_g\left(\mathbf{h}_i^{t-1} \oplus \operatorname{AGG}\left(\left\{\mathbf{h}_j^{t-1}, \forall w_j \in \mathcal{N}_{w_i}^*\right\}\right)\right)\right),
\end{equation}
where $\mathbf{h}_i^t\in \mathbb{R}^d$ is the representation of central word $w_i$ in the $t$-th layer of GNN, which is aggregated with the representation of itself $\mathbf{h}_i^{t-1}$ and its neighbors $\mathbf{h}_j^{t-1}$ in the $t-1$ layer. 
The initial representation of each word is the initialized word embedding, i.e., $\mathbf{h}_i^0 = \mathbf{v}_i$. $\sigma$ is a non-linear activation function. $W_g\in\mathbb{R}^{d\times2d}$ is the weight of a linear layer. 
$\mathcal{N}_{w_i}^*$ is the sampled neighbors. $\oplus$ is a concatenate operator. $\operatorname{AGG}$ is an aggregating function based on the attention mechanism. It aggregates the representation of neighbors with Equation~\ref{graphatt}.
\begin{equation}
\label{graphatt}
\begin{gathered}
\mathbf{q}_g^t=\sigma\left(\sum_{w_j \in \mathcal{N}_{w_i}^*} Q_g \mathbf{h}_j^{t-1}\right), \quad \mathbf{k}_j^t=\sigma\left(K_g \mathbf{h}_j^{t-1}\right) \\
a_j^t=\frac{\exp \left(\mathbf{q}_g^{t T} \boldsymbol{k}_j^t\right)}{\sum_{w_k \in \mathcal{N}_{w_i}^*} \exp \left(\mathbf{q}_g^{t^T} \boldsymbol{k}_k^t\right)}, \quad \mathbf{h}_{\mathcal{N}_{w_i}^*}^t=\sum_{w_j \in \mathcal{N}_{w_i}^*} a_j^t \mathbf{h}_j^{t-1},
\end{gathered}
\end{equation}
where $Q_g, K_g \in \mathbb{R}^{d \times d}$ is the weight of the projection layer and $a^t_j$ is the attention weight of each neighbor. The output after $T$ layers of GNN is
\begin{equation}
\label{gnn}
\begin{gathered}
\mathbf{g}_i = \mathbf{h}_i^T = \sigma(W_g(\mathbf{h}_i^{T-1}\oplus\mathbf{h}^{T-1}_{\mathcal{N}_{w_i}^*})).
\end{gathered}
\end{equation}
The central word representation $\mathbf{g}_i\in \mathbb{R}^d$ aggregated with co-click words is fused with the word-level CF signal of the word graph.

\subsubsection{Representation Alignment} In order to incorporate the word-level CF signals extracted from the word graph into the representation space of PLM, we adopt a widely used contrastive learning method to align the semantic representation of PLM $\mathbf{e}_i\in \mathbb{R}^d$ with the CF-related representation of word graph $\mathbf{g}_i\in \mathbb{R}^d$. Specifically, for a masked word $w_m$ in the input, we obtain its representations of PLM and word graph, i.e., $\mathbf{e}_m\in \mathbb{R}^d$ and $\mathbf{g}_m\in \mathbb{R}^d$. We treat them as a positive pair and treat $\mathbf{g}_i$ of other words in the same input ($i\ne m$) as negatives. We aim to pull $\mathbf{e}_m$ and $\mathbf{g}_m$ closer and push $\mathbf{e}_m$ away from other $\mathbf{g}_i$ by minimizing the following contrastive learning loss:
\begin{equation}
\label{cl}
\mathcal{L}=-\frac{1}{M} \sum_{m=1}^M \log \frac{\exp \left(\mathbf{e}_m \cdot \mathbf{g}_m / \tau\right)}{\sum_{i=0}^n \exp \left(\mathbf{e}_m \cdot \mathbf{g}_i / \tau\right)}, i\ne m,
\end{equation}
where $M$ is the number of masked words of the input item text.

It is worth noting that, during the training process, there is a parameter sharing between the word embedding of the PLM and the node embedding of the word graph. As a result, the output of a word in the PLM gradually approaches its aggregated representation of neighbor nodes in the word graph. This process results in the PLM's output containing both semantic information and word-level CF information. We refer to this recommendation-orient trained PLM as CoWPiRec.

\subsection{Downstream Recommendation}
Through constructing word graphs and pre-training on multiple domains, we obtain a text-based IRL module, CoWPiRec, that captures word-level CF signals. When transferring to a new domain, we consider two settings to evaluate the effectiveness of CoWPiRec: \textit{fine-tuning setting} and \textit{zero-shot setting}. The downstream recommendation pipeline is shown in Figure~\ref{fig_model} (c).
\subsubsection{Fine-tuning Setting}
In this setting, we train a sequential recommendation model using all training data in the new domain. Following the standard pipeline, given a user's click sequence $s=\{i_1,i_2,...,i_n\}$, for each $i_t=\{w_1,w_2,...,w_n\}$, it is fed into CoWPiRec after adding special symbols [CLS] and [SEP]. The item representation is obtained by Equation~\eqref{item_rep}.
\begin{equation}
\label{item_rep}
\mathbf{i}_t = CoWPiRec([cls; w_1; w_2; ...; w_n; sep]),
\end{equation}
where $CoWPiRec(\cdot)$ takes the representation of the [cls] position as the item representations $\mathbf{i}_t\in\mathbb{R}^d$. Then we follow~\cite{hou2022towards} and used an MoE module consisting of
multiple whitening networks to adapt the item representations and reduce the dimension, resulting $\widetilde{\mathbf{i}}_t \in \mathbb{R}^{d_V}$.

We adopt a widely used transformer network to aggregate the item representations. Specifically,  we sum the item representations and the absolute position embedding $\mathbf{p}_t\in \mathbb{R}^{d_V}$ as the input.
\begin{equation}
\mathbf{f}^0_t = \widetilde{\mathbf{i}}_t + \mathbf{p}_t.
\end{equation}
Then $\mathbf{F}^{0}=[\mathbf{f}_1^0;...;\mathbf{f}_n^0] \in \mathbb{R}^{n \times d_V}$ is fed into $L$ transformer layers, the output after $l+1$ layers is:
\begin{equation}
\mathbf{F}^{l+1} = FFN(MHAttn(F^l)).
\end{equation}
We take the $t$-th position hidden state of the last layer, i.e., $\mathbf{f}^L_n\in \mathbb{R}^{d_V}$ as the user representation $\mathbf{u}\in \mathbb{R}^{d_V}$. 

Note that since CoWPiRec already has the ability to capture recommendation signals, we don't need to update the parameters of CoWPiRec during training. Therefore we offline obtain all item representations, which significantly improves efficiency. For user representation $\mathbf{u}$, we calculate the score of candidate next item $i_{t+1}$ using the dot product:
\begin{equation}
\label{score}
score_{(i_{t+1}|s)} = Softmax(\mathbf{u} \cdot \widetilde{\mathbf{i}}_{t+1}).
\end{equation}
We use the cross-entropy loss for the next item prediction task during training. In the inference stage, we rank the items based on the dot product score.

\subsubsection{Zero-shot Setting}
In contrast to the cold-start problem, the objective of zero-shot recommendation is to determine whether a model has basic recommendation capabilities without any in-domain training. It can not be achieved with traditional ID-based recommendation models. Since the item representations generated by CoWPiRec have a remarkable semantic matching ability and could capture recommendation signals. Therefore, we directly use the nearest neighbor search with the dot product to perform the recommendation. Specifically, given all item representations in a user sequence $\{\mathbf{i}_1,\mathbf{i}_2,...,\mathbf{i}_n\}$ obtained by CoWPiRec with Equation~\eqref{item_rep}. We use mean-pooling to aggregate the item representations to obtain the user representation $\mathbf{u}$.
\begin{equation}
\mathbf{u} = \frac{1}{n}\sum_{t=1}^n\mathbf{i}_t.
\end{equation}
Then the score of the candidate item $i_{t+1}$ is calculated with Equation~\eqref {score} and we directly predict the next item according to the scores.

\subsection{Discussion}

In this section, we present the differences between our proposed CoWPiRec compared with other sequential recommendation models. 
The comparison focuses on the two components of sequential recommendation models, i.e., the IRL and SRL modules, and the model's transferable ability. 
The comparison results are shown in Table~\ref{tab:dis}.

\textbf{ID-based IRL approaches} such as SASRec~\cite{kang2018self} and BERT4Rec~\cite{sun2019bert4rec} obtain item representations with explicit item IDs. SASRec utilizes transformer layers to aggregate item ID representations and BERT4Rec performs a mask item prediction task to pre-train the bidirectional transformer layer. Since item IDs are not shared across scenarios, these approaches need to be trained from scratch when applied to new scenarios and lack transferable ability.
CoWPiRec does not rely on the item ID to perform recommendations and adopt a text-based IRL module. With the shared vocabulary across scenarios, CoWPiRec achieves transferable recommendations.

\textbf{Text-based IRL approaches} such as S\textsuperscript{3}Rec~\cite{zhou2020s3} incorporate item text representation as an auxiliary feature and perform self-supervised tasks to integrate the representation of sequence, item, and feature.
Since S\textsuperscript{3}Rec also utilizes the item id embedding, the pre-train task can only be performed in-domain. 
Different from S\textsuperscript{3}Rec, ZESRec~\cite{ding2021zero} and UniSRec~\cite{hou2022towards} purely use item text representations and perform a cross-domain pre-training on the SRL module.
The pre-trained SRL module can learn general sequence modeling patterns and contribute to the cross-scenario recommendations.
Instead of focusing only on pre-training the SRL module, MoRec~\cite{yuan2023go} train the text-based IRL and SRL module jointly with the next-item-prediction task.
We don’t pre-train the SRL module in our proposed approach and perform a word graph-based per-training task to obtain a transferable text-based IRL module, i.e., CoWPiRec.
\begin{table}[t] 
\caption{Comparison of different sequential recommenders.}
\label{tab:dis}
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{2}{c}{Used information}             & \multicolumn{2}{c}{Pre-training on}                          & \multirow{2}{*}{Transferable} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
                         & ID & Text & Item & Sequence &                               \\
\midrule
SASRec                   &    \textcolor[RGB]{0,130,130}{\CheckmarkBold}      &    \textcolor[RGB]{210,0,60}{\XSolidBrush}      &   \textcolor[RGB]{210,0,60}{\XSolidBrush}      &    \textcolor[RGB]{210,0,60}{\XSolidBrush}      &    \textcolor[RGB]{210,0,60}{\XSolidBrush}      \\
BERT4Rec                 &  \textcolor[RGB]{0,130,130}{\CheckmarkBold} &  \textcolor[RGB]{210,0,60}{\XSolidBrush}  &    \textcolor[RGB]{210,0,60}{\XSolidBrush} &    \textcolor[RGB]{0,130,130}{\CheckmarkBold}          &     \textcolor[RGB]{210,0,60}{\XSolidBrush}                \\
S3Rec                    & \textcolor[RGB]{0,130,130}{\CheckmarkBold} & \textcolor[RGB]{0,130,130}{\CheckmarkBold}     &    \textcolor[RGB]{210,0,60}{\XSolidBrush}  & \textcolor[RGB]{0,130,130}{\CheckmarkBold}    &     \textcolor[RGB]{210,0,60}{\XSolidBrush}           \\
ZESRec                   & \textcolor[RGB]{210,0,60}{\XSolidBrush} &  \textcolor[RGB]{0,130,130}{\CheckmarkBold}   &    \textcolor[RGB]{210,0,60}{\XSolidBrush}       &  \textcolor[RGB]{0,130,130}{\CheckmarkBold}        &   \textcolor[RGB]{0,130,130}{\CheckmarkBold}             \\
UniSRec                  & \textcolor[RGB]{210,0,60}{\XSolidBrush} &  \textcolor[RGB]{0,130,130}{\CheckmarkBold}  &   \textcolor[RGB]{210,0,60}{\XSolidBrush}     &    \textcolor[RGB]{0,130,130}{\CheckmarkBold}      &      \textcolor[RGB]{0,130,130}{\CheckmarkBold}        \\
MoRec                  & \textcolor[RGB]{210,0,60}{\XSolidBrush} &  \textcolor[RGB]{0,130,130}{\CheckmarkBold}  &   \textcolor[RGB]{0,130,130}{\CheckmarkBold}     &    \textcolor[RGB]{0,130,130}{\CheckmarkBold}      &      \textcolor[RGB]{0,130,130}{\CheckmarkBold}        \\
\midrule
CoWPiRec                   & \textcolor[RGB]{210,0,60}{\XSolidBrush} &  \textcolor[RGB]{0,130,130}{\CheckmarkBold}  &  \textcolor[RGB]{0,130,130}{\CheckmarkBold}        &  \textcolor[RGB]{210,0,60}{\XSolidBrush}          &  \textcolor[RGB]{0,130,130}{\CheckmarkBold}    \\
\bottomrule
\end{tabular}
\end{table}

==> tables/data2.tex <==
\begin{tabularx}{\textwidth}{l l l l X}
\toprule
Name & Link & Modalities & Domain & Notes \\
\midrule
ReDial & \href{https://github.com/ReDialData/website}{github} & T & Movies & Conversational recommendation (\cite{redial}) \\
Microlens & \href{https://github.com/westlake-repl/MicroLens}{github} & A, I, T, V & Movies & MovieLens with micro-reviews (\cite{microlens}) \\
Netflix Prize dataset  & \href{https://www.kaggle.com/datasets/netflix-inc/netflix-prize-data}{kaggle} & C, T & Movies/Series & old one: \cite{netflixprize} \\
Netflix & \href{https://github.com/HKUDS/PromptMM}{github} & C, I, N, T & Movies/Series & They adapted existing datasets into multimodal (\cite{promptmm}) \\
MovieLens (augmented) & \href{https://github.com/HKUDS/PromptMM}{github} & C, I, N, T & Movies/Series & They adapted existing datasets into multimodal (\cite{promptmm}) \\
Douban  & \href{https://github.com/fengzhu1/GA-DTCDR}{github} & C, I, N, T & Multi-domain & ~ \\
U-NEED  & \href{https://github.com/LeeeeoLiu/U-NEED}{github} & C, G, T & Multi-domain & Includes 7.7k annotated dialogues, 333k user actions, and 332k product tuples; dialog-based \\
Tenrec & \href{https://tenrec0.github.io}{Link} & B, C, T & Multi-domain & Large-scale benchmark with positive and negative feedback across 4 scenarios. New: \cite{tenrec} \\
NetEase Cloud Music & \href{https://ssrn.com/abstract=3554826}{joining INFORMS RMP} & A, C, I, N, T & Music & 57M+ impressions; short music video cards, user behaviors, and creator/content/user metadata. \\
Coat & \href{https://www.cs.cornell.edu/~schnabts/mnar/}{Lin}k & T & Music & Version of Netflix curated for MNAR studies; alignment with MovieLens (\cite{coat}) \\
MSD & \href{http://millionsongdataset.com/challenge}{Link} & A, T & Music & \cite{deepmultimodal} \\
LFM & \href{ https://www.heywhale.com/mw/dataset/5cfe0526e727f8002c36b9d9/content}{Link} & A, I, T & Music & Likely LastFM (\cite{LastFM}) \\
MM-Rec  & \href{https://github.com/zcfinal/MM-Rec}{github} & I, T & News & \cite{MM_Rec} \\
TianchiNews & \href{https://tianchi.aliyun.com/competition/entrance/531842/introduction}{Link in Chinese} & T & News & ~ \\
MIND & \href{https://msnews.github.io}{github} & T & News & Microsoft News clicks (paper: \cite{mind}) \\
Yelp & \href{https://www.yelp.com/dataset}{Link} & I, POI, T & POI & ~ \\
Kwai & \href{https://zenodo.org/records/4023390#.Y9YZ6XZBw7c}{Link} & I, T, V & Short video & \cite{kwai} \\
TikTok & \href{https://jianxinma.github.io/disentangle-recsys.html}{github}, \href{https://www.kaggle.com/datasets/yasaminjafarian/tiktokdataset}{kaggle}, \href{https://drive.google.com/file/d/1dmZh6I3kvh__nB-nWL8VT3jIn3mDL1VA/view}{drive} & A, I, T, V & Short video & ~ \\
Microlens (New) & \href{https://recsys.westlake.edu.cn/MicroLens-50k-Dataset}{Link} & A, I, T, V & Short video & Includes MicroLen with raw video, audio, cover images, titles, and video comments. New: \cite{microlens} \\
NineRec  & \href{https://github.com/westlake-repl/NineRec}{github} & C, I, T & Short video & High-res cover images and descriptive texts for 400k+ items across 9 platforms. New: \cite{ninerec} \\
KuaiSAR & \href{https://kuaisar.github.io/}{Link} & B, C, T & Short video & \cite{KuaiSAR} \\
WeChat5D & \href{https://github.com/yaqingwang/WeFEND-AAAI20}{github} & C, I, N, T & Social Media & WeChat fake news dataset with user behavior and image-text pairs. \\
Pinterest  & \href{https://github.com/edervishaj/pinterest-recsys-dataset?tab=readme-ov-file}{github} & I, T & Social Media & \cite{pinterest} \\
MM-INS  & \href{https://github.com/w5688414/AMNN}{github} & I, T & Social Media & \cite{mm_ins} \\
TripAdvisor & \href{https://www.kaggle.com/datasets/andrewmvd/trip-advisor-hotel-reviews}{kaggle} & T & Travel / Hotels & Contains hotel reviews and ratings; often used for sentiment-aware or text-based recommendation tasks  \\
YT8M-MusicVideo & \href{https://research.google.com/youtube8m}{Link} & T, V & Video & Includes pre-extracted audio-visual features and metadata (e.g. titles, tags) from YouTube videos  \\
\bottomrule
\end{tabularx}

==> tables/main_table.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{Paper Title} & \textbf{LLM Methods} & \textbf{Prompting (Hard Prompting)} & \textbf{Prompting (Soft Prompting)} & \textbf{Training (Fine-tuning/LoRA/Adapters)} & \textbf{Training (Black-box/Encoder)} & \textbf{Training (Masking Conversion)} & \textbf{Training (Pretrained MLLMs)} & \textbf{Data Type Adaptation (KG Conversion)} & \textbf{Data Type Adaptation (Code Conversion)} & \textbf{Data Type Adaptation (Other Conversions)} & \textbf{Disentangle} & \textbf{Disentangle Encoder} & \textbf{Attention Methods} & \textbf{VAE Methods} & \textbf{Alignment (CL Alignment)} & \textbf{Alignment (Encoder)} & \textbf{Involved Graphs (User-Item Graph)} & \textbf{Involved Graphs (Inter-Items and Inter-Users)} & \textbf{Involved Graphs (External Knowledge Graph)} & \textbf{Fusion Classification (Location of Fusion)} & \textbf{Fusion Classification (Early Fusion)} & \textbf{Fusion Classification (Intermediate Fusion)} & \textbf{Fusion Classification (Late Fusion)} & \textbf{Fusion Classification (Type of Fusion)} & \textbf{Fusion Classification (Coarse-Grained Fusion)} & \textbf{Fusion Classification (Fine-Grained Fusion)} & \textbf{No LLM-Related Classification (Datasets)} & \textbf{No LLM-Related Classification (Metrics)} & \textbf{No LLM-Related Classification (Tasks and Models)} \\
\hline
Example Paper & Yes/No & Yes/No & Yes/No & Yes/No & Yes/No & Yes/No & Yes/No & Yes/No & Yes/No & Yes/No & Yes/No & Yes/No & Yes/No & Yes/No & Yes/No & Yes/No & Yes/No & Yes/No & Yes/No & Yes/No & Yes/No & Yes/No & Yes/No & Yes/No & Yes/No & Yes/No & Yes/No & Yes/No & Yes/No \\
\hline
\end{tabular}
\caption{Paper Classification Table}
\label{tab:paper_classification}
\end{table}

